LLM Augmentations to support Analytical Reasoning over Multiple Documents

Building on their demonstrated ability to perform a variety of tasks, we investigate the application of large language models (LLMs) to enhance in-depth analytical reasoning within the context of intelligence analysis. Intelligence analysts typically work with massive dossiers to draw connections between seemingly unrelated entities, and uncover adversaries' plans and motives. We explore if and how LLMs can be helpful to analysts for this task and develop an architecture to augment the capabilities of an LLM with a memory module called dynamic evidence trees (DETs) to develop and track multiple investigation threads. Through extensive experiments on multiple datasets, we highlight how LLMs, as-is, are still inadequate to support intelligence analysts and offer recommendations to improve LLMs for such intricate reasoning applications.

==> sections/algorithm_2.tex <==
\begin{figure}[h]
\begin{minipage}{\columnwidth}
    \begin{algorithm}[H]
    \scriptsize
    \caption{\merge}
    \label{algo:merge}
    \begin{algorithmic}[1]
    \Require $\mathit{DOT}$
    
    \Function{Retrieve}{$DOT_{query}$}
        \State Vector Search in $DETs$
    \EndFunction
    
    \Function{LLM based Filtering}{$DOT_{candidates}$, $DOT_{query}$}
        \State Invoke $\mathcal{LLM}$
    \EndFunction
    
        \State $DOT_{candidates} \gets \Call{Retrieve}{DOT}$
        \State $DOT_{filtered} \gets \Call{LLM based Filtering}{DOT_{candidates}, DOT_{query}}$
        \If{$|DOT_{filtered}|\neq \emptyset$} 
            \State $DOTs_{candidates} \gets \Call{Hypo. Node Consolidation}{DOTs_{filtered}}$
            \State $DOTs_{candidates} \gets \Call{Evid. Node Collection}{DOTs_{candidates}}$
            \State $DOT_{new} \gets $ Invoke $\mathcal{LLM}$
            \State \Call{\merge\ref{algo:merge}}{$DOT_{new}$}
            \State \Call{\db}{$DOT_{new}$}
        \EndIf
            
    \end{algorithmic}
    \end{algorithm}
\end{minipage}%
\end{figure}

==> sections/diff_models_table.tex <==
\begin{table*}[t]
    \centering
        \caption{ROUGE and METEOR scores on three datasets for different LLMs}
        \label{tab:diff_models}
        \resizebox{0.8\textwidth}{!}{%
        \begin{tabular}{@{}lrrrrrrrrrrrr@{}}
        \toprule
        \textbf{}      & \multicolumn{4}{c}{\textbf{Crescent}} & \multicolumn{4}{c}{\textbf{Atlantic Storm}} & \multicolumn{4}{c}{\textbf{Manpad}} \\ \midrule
        \textbf{Model} & METEOR    & R1      & R2     & RL     & METEOR     & R1       & R2       & RL       & METEOR   & R1     & R2     & RL     \\ \midrule
        GPT-3.5        & 0.23      & 0.16    & 0.04   & 0.13   & 0.28       & 0.22     & 0.05     & 0.17     & 0.30     & 0.09   & 0.22   & 0.30   \\
        GPT-4          & 0.31      & 0.21    & 0.07   & 0.17   & 0.26       & 0.28     & 0.06     & 0.18     & 0.31     & 0.21   & 0.09   & 0.32   \\
        Llama-2        & 0.20      & 0.19    & 0.03   & 0.11   & 0.21       & 0.21     & 0.03     & 0.15     & 0.28     & 0.36   & 0.08   & 0.26   \\
        Mistral-7B        & 0.26      & 0.23    & 0.07   & 0.16   & 0.25       & 0.20     & 0.04     & 0.15     & 0.34     & 0.37   & 0.11   & 0.26   \\
        Gemma-2        & 0.17      & 0.08    & 0.03   & 0.07   & 0.15       & 0.07     & 0.02     & 0.05     & 0.27     & 0.18   & 0.07   & 0.15   \\ \bottomrule
        \end{tabular}%
        }
\end{table*}
